DeepView: Visualizing Classification Boundaries of Deep Neural Networks as Scatter Plots Using Discriminative Dimensionality Reduction

Machine learning algorithms using deep architectures have been able to implement increasingly powerful and successful models. However, they also become increasingly more complex, more difficult to comprehend and easier to fool. So far, most methods in the literature investigate the decision of the model for a single given input datum. In this paper, we propose to visualize a part of the decision function of a deep neural network together with a part of the data set in two dimensions with discriminative dimensionality reduction. This enables us to inspect how different properties of the data are treated by the model, such as outliers, adversaries or poisoned data. Further, the presented approach is complementary to the mentioned interpretation methods from the literature and hence might be even more useful in combination with those. Code is available at https://github.com/LucaHermes/DeepView .

==> suppl1.tex <==



\begin{lemma}
    Let $S$ be a finite dimensional real vector space. Let $d : S \times S \to \R$ be a metric induced by an inner product and $X$ be a $S$-valued random variable. Then it holds
    \begin{align*}
    \argmin_{x \in S} \E\left[ d(X,x)^2 \right] &= \argmin_{x \in S} \E\left[ \Vert X - x \Vert_2^2 \right].
    \end{align*}
    \begin{proof}
        Since $d$ is induced by an inner product we may find a matrix $A$ such that $d(x,y)^2 = (x-y)^tA(x-y)$. 
        
        \textbf{1. Case $A$ is a diagonal matrix: } Then it holds
        \begin{align*}
        \E\left[ d(X,x)^2 \right] &= \sum_i a_{ii} \E\left[(X_i - x_i)^2\right]
        \end{align*}
        since we may optimize each component of $x$ separately the statement follows.
        
        \textbf{2. Case $A$ is not diagonal: } Using the spectral theorem we obtain $A = U^tDU$ (by spectral theorem we obtain $A = VDV^t$ then we define $U = V^t$, since $V$ is unitary so is $U$), where $D$ is a diagonal matrix an $U$ is unitary. Hence it follows
        \begin{align*}
        \argmin_{x \in S} \E\left[ d(X,x)^2 \right] 
        &=\argmin_{x \in S} \E\left[ (U(X-x))^tD(U(X-x)) \right] 
        \\&=\argmin_{x \in S} \E\left[ (UX-Ux)^tD(UX-Ux) \right] 
        \\&=U^{-1} \argmin_{x' \in \im U} \E\left[ (UX-x')^tD(UX-x') \right] 
        \\&=U^{-1}\argmin_{x' \in \im U} \E\left[ \Vert UX - x'\Vert_2^2 \right] & \text{1. Case}
        \\&=\argmin_{x \in S} \E\left[ \Vert UX-Ux \Vert_2^2 \right] 
        \\&=\argmin_{x \in S} \E\left[ \Vert U(X-x) \Vert_2^2 \right] 
        \\&=\argmin_{x \in S} \E\left[ \Vert X-x\Vert_2^2 \right]. & \text{$U$ is unitary}
        \end{align*}
    \end{proof}
\end{lemma}

\begin{remark}[Derivation of $\piinv$]
It holds
\begin{align*}
\piinv(\y) &:= \argmin_{\x \in S} \sum_{i = 1}^n D(p_i(\y)||q_i(\x)) \overset{!}{=} \argmin_{\x \in S} \sum_{i = 1}^n H(p_i(\y);q_i(\x)) 
\end{align*}
since $\frac{\partial}{\partial \theta} D_\KL (X \Vert f_\theta(Y) ) = \frac{\partial}{\partial \theta} (H(X ; f_\theta(Y)) - H(X)) = \frac{\partial}{\partial \theta} H(X ; f_\theta(Y))$, where $H(\cdot)$ denotes entropy and $H(\cdot;\cdot)$ denotes the cross entropy. Now by plugging in the definitions and approximations we obtain
\begin{align*}
H(\y;\x) &= -\sum_{i = 1}^n w_i(\y) \log v_i(\x) \underbrace{-\sum_{i = 1}^n (1-w_i(\y))\log (1-v_i(\x))}_{\approx 0} \\&= -\sum_{i = 1}^n w_i(\y) \left(- \frac{\Vert \x - \s_i \Vert_2^2}{\sigma_i} \right) \\&= \sum_{i = 1}^n \frac{w_i(\y)}{\sigma_i} \Vert \x -  \s_i \Vert_2^2 
\\\Rightarrow \nabla_\x H(\y;\x) &= 2 \sum_{i = 1}^n \frac{w_i(\y)}{\sigma_i} (\x - \s_i) \overset{!}{=} 0
\\\Leftrightarrow \x &= \frac{\sum_{i = 1}^n \frac{w_i(\y)}{\sigma_i} \s_i }{\sum_{i = 1}^n \frac{w_i(\y)}{\sigma_i}}.
\end{align*}
Furthermore using the lemma above we see that
\begin{align*}
    \x^*
      &= \argmin_{\x \in S} -\sum_{i = 1}^n w_i(\y) \log v_i(\x) 
    \approx \argmin_{\x \in S} \sum_{i = 1}^n \frac{w_i(\y)}{\sigma_i} d_{s^*}(\x,\s_i)^2
    \\&= \argmin_{\x \in S} C \sum_{i = 1}^n \frac{\frac{w_i(\y)}{\sigma_i}}{C} d_{s^*}(\x,\s_i)^2
    = \argmin_{\x \in S} C \E_P[ d_{s^*}(\x,X)^2 ]
    \\&= \argmin_{\x \in S} C \E_P[ \Vert \x - X \Vert^2 ]
    =\argmin_{\x \in S} C \sum_{i = 1}^n \frac{\frac{w_i(\y)}{\sigma_i}}{C} \Vert \x - \s_i \Vert^2
    \\&= \frac{\sum_{i = 1}^n\frac{w_i(\y) \s_i}{\sigma_i}}{\sum_{i = 1}^n\frac{w_i(\y)}{\sigma_i}},
\end{align*}
where $C = \sum_{i = 1}^n\frac{w_i(\y)}{\sigma_i}$, $d_{s^*}$ the approximation of $d_S$ at ${s^*}$, $X : \{1,...,n\} \to , i \mapsto \s_i$ a random variable and $P(I) = \frac{1}{C} \sum_{i \in I} \frac{w_i(\y)}{\sigma_i}$.
\end{remark}

\begin{lemma}[Derivation of $\eta_\textnormal{opt}$]
Let $R,S$ be finite dimensional, real vector spaces. Let $\r_i \in R,\s_i \in S,A_i \in \textnormal{Mat}_\R(S,S), \; i = 1,...,n$ and $\Theta,J \in \textnormal{Mat}_\R(R,S)$. Assume that $A_i$ are symmetric and positive definite and denote by $\Vert \cdot \Vert_i$ the induced norm, i.e. $\Vert s \Vert_i := \sqrt{s^t A_i s}$. Then it holds
\begin{align*}
\argmin_{\eta} \sum_{i = 1}^n \Vert (\Theta-\eta J) \r_i - \s_i \Vert_i^2 = \frac{\sum_{i = 1}^n (\Theta \r_i - \s_i)^t A_i J \r_i }{\sum_{i = 1}^n \r_i^t J^t A_i J \r_i }.
\end{align*}
\begin{proof}
It holds
\begin{align*}
\frac{\d}{\d \eta} \sum_{i = 1}^n \Vert (\Theta-\eta J) \r_i - \s_i \Vert_i^2 
&= 2 \sum_{i = 1}^n ((\Theta-\eta J) \r_i - \s_i)^t A_i J \r_i \overset{!}{=} 0 \\
\Leftrightarrow \sum_{i = 1}^n (\Theta \r_i - \s_i)^t A_i J \r_i &= \eta \sum_{i = 1}^n \r_i^t J^t A_i J \r_i
\end{align*}
\end{proof}
\end{lemma}

\begin{algorithm}
    \caption{Construction of Delaunay neighborhood}
    \label{ConstTriaN}
    \begin{algorithmic}[1]
        \Procedure{ConstructDelaunayNeighborhood}{$(r_i)_{i=1,...,n}$ data points, $n_s$ number of simplices, $n_k$ number of neighbors, $\varepsilon$ minimal border distance}
        \State $C \gets \Call{K-Means}{(r_i)_i,n_s}$\;
        \State $B \gets \Call{Border}{(r_i)_i, \varepsilon}$\;
        \Comment{Vertices of a rectangle containing $\cup_i B_{r_i}(\varepsilon)$}
        \State $V \gets C \cup B$\;
        \Comment{Assure that every $r_i$ is actually contained in one simplex}
        \State $S \gets \Call{DelaunayTriangulation}{V}$\;
        \Comment{Delaunay triangulation for $V$, returns set of simplices}
        \For{$i \in [1,|S|]_\N$}
        \State $V' \gets \Call{GetVertices}{S_i}$\;
        \Comment{Vertices of $S_i$} 
        \For{$j \in [1,D+1]_\N$}
        \State $\nu_j \gets \Call{NearestNeighbors}{(r_i)_i, V'_j, n_k}$\;
        \Comment{$n_k$ nearest neighbors of $V'_j$ in $(r_i)_i$ sorted by distance}
        \EndFor
        \State $N_i \gets \Call{ComposeNeighbors}{\nu , n_k}$
        \EndFor
        \State \textbf{return} $S, N$ 
        \Comment{Delaunay triangulation $S$, Delaunay neighborhood $N$}
        \EndProcedure
        
        \Procedure{ComposeNeighbors}{$(N_{ij})_{i=1,...,n,\;j=1,...,n_k}$ 2d-array of nearest neighbors; row wise sorted by distance, $n_k$ number of neighbors}
        \For{$i \in [1,n]_\N$}
        \State $k_i \gets 0$ 
        \EndFor
        \State $D \gets \emptyset$ \;
        \Comment{Use a heap for speedup}
        \State $j \gets 1$\;
        \State $i \gets 1$ \;
        \While{$j \leq n_k$}
        \State $k_i \gets k_i +1$ \;
        \If{$N_{ik_i} \not\in D$}
        \Comment{$N_{ik_i}$ is not already contained in $C$}
        \State $D \gets D \cup \{N_{ik_i}\}$\;
        \State $C_j \gets N_{ik_i}$ \;
        \State $i \gets (i \mod n)+1$ \;
        \State $j \gets j+1$ \;
        \EndIf
        \EndWhile
        \State \textbf{return} $C$ 
        \Comment{composed neighborhood}
        \EndProcedure   
    \end{algorithmic}
\end{algorithm}

==> suppl2.tex <==


\begin{figure}
  \centering
  \includegraphics[width=0.49\linewidth]{imagenet_classifVis_annotated}
  \includegraphics[width=0.5\linewidth, trim= 0mm 0mm 0mm 0mm]{imagenet_invExamples}
  \caption{A visualization of a part of ImageNet and the AlexNet network together with markers of specified positions around the adversarial example (left). The resulting images of the inverse mapping $\piinv$ for the previously specified positions, together with the assigned label and according certainty of the classifier (right).}
  \label{fig:imagenet}
\end{figure}


For our current experiments we utilize a subset of three classes from the full ImageNet data set,\footnote{http://image-net.org/} the classes 'acoustic guitar', 'electric guitar' and 'grand piano'. 
As the pre-trained model we choose the popular AlexNet \cite{alexnet} and apply DeepView to 300 randomly selected data points and one adversarial example. 

The resulting visualization is shown in \fig\ \ref{fig:imagenet} with additional white circles around points for which the $\piinv$ mapping is inaccurate (i.e.\ where $\Qd$ counts mistakes). The evaluation is summarized in \tab\ \ref{tab:eval_res} and reveals lower scores as compared to the CIFAR-10 dataset. This is not surprising because the dataset, as well as the classifier (being trained on 1000 classes), is much more complex. Furthermore, the scores do not consider a top-5 measure as partially common with this dataset.

Concerning the visualization, we can observe that the 'piano' class is further away from the other two and that a set of points is classified as 'other' and is positioned in the middle. 
Again, the adversarial example is positioned outside of the main cluster and we investigate the area around it in the same as previously. While the position '0' is mapped to an image which is classified properly, the images of '1' to '5' are predicted with a high uncertainly and partially even wrong, although showing clearly guitars. 

We select two further areas close to points being outside of their main cluster and mark them with '6' and '7'. This way we can get an impression why these images are classified incorrectly. In this case, the images show multiple objects with the target object being partially rather in the background.


